Plane Graphs are Facially-non-repetitively $10^{4 \cdot10^7}$-Choosable

A sequence $\left(x_1,x_2,\ldots,x_{2n}\right)$ of even length is a repetition if $\left(x_1,\ldots,x_n\right) = \left(x_{n+1},\ldots,x_{2n}\right)$. We prove existence of a constant $C < 10^{4 \cdot 10^7}$ such that given any planar drawing of a graph $G$, and a list $L(v)$ of $C$ permissible colors for each vertex $v$ in $G$, there is a choice of a permissible color for each vertex such that the sequence of colors of the vertices on any facial simple path in $G$ is not a repetition.

==> fig_main.tex <==
\begin{figure}[h]
  \begin{center}
\begin{tikzpicture}[>=latex]
\end{tikzpicture}
\missingfigure{}
\end{center}
\caption{
  Auxiliary graph on the faces.
}
\label{fig:main}
\end{figure}

